Forecastable Component Analysis (ForeCA)

I introduce Forecastable Component Analysis (ForeCA), a novel dimension reduction technique for temporally dependent signals. Based on a new forecastability measure, ForeCA finds an optimal transformation to separate a multivariate time series into a forecastable and an orthogonal white noise space. I present a converging algorithm with a fast eigenvector solution. Applications to financial and macro-economic time series show that ForeCA can successfully discover informative structure, which can be used for forecasting as well as classification. The R package ForeCA (http://cran.r-project.org/web/packages/ForeCA/index.html) accompanies this work and is publicly available on CRAN.

==> arxiv_load_packages.tex <==
%\usepackage{float}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
%\usepackage{lineno} 

\usepackage{amssymb, amsmath, amscd}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{verbatim}
%\usepackage{subfig}
%\usepackage{epstopdf}

\usepackage{algorithm}
\usepackage[noend]{algorithmic}
%\usepackage{diagxy}
\usepackage{tikz}
\usetikzlibrary{shapes,arrows, fadings, calc, positioning}

%\usepackage{fancyhdr}
%\usepackage{setspace}
\usepackage{url}
%\usepackage{enumitem}
\usepackage{enumerate}

\usepackage{paralist} % for inline list; e.g. here i) is this and ii) that (no line break)
\usepackage{caption}
\DeclareCaptionType{copyrightbox}
\usepackage{subcaption}
